WayTrace: A Map-to-Language-to-Trace Hierarchy for Embodied Urban Navigation

Web services provide walking directions for nearly every city, but following them reliably over long routes remains challenging for autonomous robots. Point-goal navigation policies rely heavily on accurate GNSS, while most vision-language navigation models struggle to execute even short instructions outdoors. We present WayTrace, a hierarchical system that connects web-map directions to robot motion through language. An off-the-shelf orchestrator vision-language model reads the turn-by-turn directions, a satellite map and recent camera images, and issues one atomic language command at a time, such as "cross the road to the left". An onboard trace predictor, trained on over one million automatically labelled samples from street-level images, draws the path for this command in the image, and a reinforcement learning policy tracks it. In long-range simulated missions, WayTrace remains robust to GNSS noise and rarely leaves crosswalks or sidewalks, while point-goal baselines degrade sharply with about ten times more violations. Deployed on a wheeled-legged robot, WayTrace completes real-world missions of up to 1.37 km at about 1.1 m/s through a busy city centre, rural trails and a university campus, handling crosswalks, staircases and construction sites. Project page: https://way-trace.github.io

==> tables/exp1_openloop.tex <==
\textbf{Ours} & \textbf{83.2} & \textbf{85.8} & \textbf{5.0} & \textbf{4.0} & \textbf{97.9} & \textbf{98.3} & \textbf{70.4} & \textbf{72.5} & \textbf{8.6} & \textbf{7.5} & \textbf{92.6} & \textbf{94.8} \\
CityWalker$^\dagger$ & 57.0 & 66.2 & 13.9 & 10.0 & 90.4 & 91.2 & 50.9 & 60.7 & 15.8 & 11.4 & 87.3 & 87.2 \\
VAMOS$^\dagger$ & 56.6 & 42.6 & 16.4 & 19.8 & 97.7 & 95.5 & 48.8 & 33.7 & 18.5 & 22.3 & 92.5 & 91.6 \\
Foresight & 50.5 & 68.3 & 15.0 & 8.9 & 77.4 & 90.5 & 41.8 & 60.1 & 17.3 & 10.9 & 75.1 & 89.2 \\
VENTURA & 45.2 & 60.4 & 17.1 & 11.9 & 65.6 & 67.8 & 33.2 & 48.5 & 20.2 & 14.7 & 70.2 & 75.2 \\
TIC-VLA & 22.6 & 44.6 & 26.6 & 19.3 & 66.3 & 72.0 & 10.5 & 32.8 & 29.8 & 22.1 & 80.3 & 85.6 \\


==> tables/exp4b_vlm.tex <==
Qwen3.8-Flash-Next (ours, self-hosted) & 5.1 & 4.3 & 6.1 & 0\,/\,200 & 18\,/\,338 & 20\,/\,244 & 2\,/\,66 & 9\,/\,87 & 0\,/\,22 & 1.38 & local \\
Gemini 3.5 Flash-Lite & 5.9 & 4.0 & 8.2 & 4\,/\,200 & 19\,/\,338 & 5\,/\,244 & 0\,/\,66 & 28\,/\,87 & 0\,/\,22 & 5.12 & \$2.9 \\
Gemini 3.8 Flash & \textbf{3.2} & 3.2 & \textbf{3.3} & 0\,/\,200 & 10\,/\,338 & 4\,/\,244 & 12\,/\,66 & 5\,/\,87 & 0\,/\,22 & 6.53 & \$7.4 \\
GPT-6 Sol & \textbf{3.2} & \textbf{1.5} & 5.4 & 2\,/\,200 & 15\,/\,338 & 6\,/\,244 & 1\,/\,66 & 7\,/\,87 & 0\,/\,22 & 4.52 & \$7.1 \\


==> tables/exp4b_vlm_compact.tex <==
Qwen3.8-Flash-Next (ours) & 5.1 & 4.3 & 6.1 & \textbf{1.4} & --- \\
Gemini 3.5 Flash-Lite & 5.9 & 4.0 & 8.2 & 5.1 & 2.9 \\
Gemini 3.8 Flash & \textbf{3.2} & 3.2 & \textbf{3.3} & 6.5 & 7.4 \\
GPT-6 Sol & \textbf{3.2} & \textbf{1.5} & 5.4 & 4.5 & 7.1 \\


==> tables/supp_failures.tex <==
CityWalker & 0 & 30 & \textcolor{black!35}{0} & \textcolor{black!35}{0} & 2 & 4 & \textcolor{black!35}{0} & \textcolor{black!35}{0} & 18 & \textcolor{black!35}{0} & \textcolor{black!35}{0} & 24 \\
\addlinespace[2pt]
VAMOS & 0 & 30 & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & 1 & \textcolor{black!35}{0} & \textcolor{black!35}{0} & 25 & \textcolor{black!35}{0} & \textcolor{black!35}{0} & 26 \\
\addlinespace[2pt]
CityWalker + RL policy & 0 & 30 & 16 & \textcolor{black!35}{0} & \textcolor{black!35}{0} & 3 & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & 19 \\
CityWalker + RL policy & 2 & 30 & 10 & 2 & \textcolor{black!35}{0} & 4 & \textcolor{black!35}{0} & \textcolor{black!35}{0} & 2 & \textcolor{black!35}{0} & \textcolor{black!35}{0} & 18 \\
CityWalker + RL policy & 5 & 30 & 8 & 1 & \textcolor{black!35}{0} & 3 & 6 & 2 & 3 & 1 & \textcolor{black!35}{0} & 24 \\
CityWalker + RL policy & 7 & 30 & 4 & \textcolor{black!35}{0} & 1 & 4 & 9 & \textcolor{black!35}{0} & 5 & \textcolor{black!35}{0} & \textcolor{black!35}{0} & 23 \\
\addlinespace[2pt]
VAMOS + RL policy & 0 & 30 & 9 & 2 & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & 11 \\
VAMOS + RL policy & 2 & 30 & 11 & 1 & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & 12 \\
VAMOS + RL policy & 5 & 30 & 5 & 6 & 1 & 5 & 3 & 1 & 2 & 2 & \textcolor{black!35}{0} & 25 \\
VAMOS + RL policy & 7 & 30 & 2 & 3 & 2 & 7 & 6 & 1 & 2 & 4 & \textcolor{black!35}{0} & 27 \\
\addlinespace[2pt]
\method & 0 & 30 & \textcolor{black!35}{0} & \textcolor{black!35}{0} & 1 & \textcolor{black!35}{0} & \textcolor{black!35}{0} & 1 & \textcolor{black!35}{0} & 3 & \textcolor{black!35}{0} & 5 \\
\method & 2 & 30 & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & 1 & 5 & \textcolor{black!35}{0} & 6 \\
\method & 5 & 30 & 1 & \textcolor{black!35}{0} & \textcolor{black!35}{0} & 1 & \textcolor{black!35}{0} & \textcolor{black!35}{0} & 1 & 5 & \textcolor{black!35}{0} & 8 \\
\method & 7 & 30 & 1 & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & 1 & 1 & 8 & \textcolor{black!35}{0} & 11 \\
\addlinespace[2pt]
\method, oracle orchestrator & 0 & 30 & 2 & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & \textcolor{black!35}{0} & 1 & \textcolor{black!35}{0} & 3 \\


==> tables/supp_missions.tex <==
M1 & \anon{A}{Neumarkt} & Rheinfelder Bierhaus & 152 & 1 turn & 0 & 669 \\
M2 & \anon{B}{Bellevue} & Karl der Grosse & 223 & 1 turn & 0 & 858 \\
M3 & \anon{C}{Mühlesteg} & dieci pizza takeaway & 328 & 4 turns, 2 crossings & 2 & 1119 \\
M4 & \anon{C}{Mühlesteg} & Burger King & 361 & 2 turns, 3 crossings & 3 & 1195 \\
M5 & \anon{D}{Seilergraben} & Burger King & 393 & 1 fork, 2 crossings, stairs down & 3 & 1275 \\
M6 & \anon{D}{Seilergraben} & Café Zähringer & 406 & 2 crossings & 2 & 1308 \\
M7 & \anon{A}{Neumarkt} & Starbucks & 518 & 2 turns, 1 crossing & 1 & 1596 \\
M8 & \anon{B}{Bellevue} & Café Henrici & 633 & 1 turn & 0 & 1881 \\
M9 & \anon{E}{Zunfthaus zur Waag} & dieci pizza takeaway & 799 & 1 turn, 1 fork, 2 crossings & 2 & 2289 \\
M10 & \anon{F}{Limmatquai, Central} & Karl der Grosse & 864 & 2 turns, 2 crossings & 3 & 2461 \\
\midrule
\multicolumn{3}{l}{Total} & 4676 & 14 turns, 2 forks, 14 crossings, 1 staircase & 16 & \\

